cozy: Comparative Symbolic Execution for Binary Programs

This paper introduces cozy, a tool for analyzing and visualizing differences between two versions of a software binary. The primary use case for cozy is validating "micropatches": small binary or assembly-level patches inserted into existing compiled binaries. To perform this task, cozy leverages the Python-based angr symbolic execution framework. Our tool analyzes the output of symbolic execution to find end states for the pre- and post-patched binaries that are compatible (reachable from the same input). The tool then compares compatible states for observable differences in registers, memory, and side effects. To aid in usability, cozy comes with a web-based visual interface for viewing comparison results. This interface provides a rich set of operations for pruning, filtering, and exploring different types of program data.

==> sections/acknowledgments.tex <==
%% if specified like this the section will be committed in review mode
\acknowledgments{
Acknowledge DARPA grant stuff}

==> sections/background.tex <==
% TODO: A short intro to symbolic execution and how angr works. An intro to concolic execution. Intro how symbolic execution can be visualized as a branching tree.

\toolname{} compares binaries by computing all possible paths through a binary pre- and
post-patch, and then determining which paths have changed, and in what ways they
have changed. How is it possible to compute all possible paths through a binary?

When a program is evaluated, it can be thought of as performing various
operations, transforming an initial program state (e.g. a configuration of
memory and register contents, or a set of assignments to variables) into a final
program state, via a sequence of intermediate states. \emph{Symbolic execution}
is the practice of computing the constraints on possible final and intermediate
program states, in terms of features of the initial program
state.\footnote{
  Modern symbolic execution tools include KLEE \cite{KLEE},
  Verifast \cite{Verifast}, SymQEMU \cite{SymQEMU}, and Angr \cite{ANGR}.
  Foundational work in the area dates back to at least 1975, notably with King
  \cite{EFFIGY} and Boyer et al. \cite{SELECT}. \hl{cite canonical stuff eg
  KLEE}.
}

For example, we might consider a trivial program that increments a variable twice:
\begin{algorithm}
  input:   An Integer $x_I$, assigned to X.
  output:  None
  begin
    X $\leftarrow$ X+1
    X $\leftarrow$ X+1
    return
  end
\end{algorithm}
Given a concrete assignment to X, say $2$, we know that at the end of the
program, $\textrm{X} = 4$. More generally, no matter how we assign to the input
variable, we know the at the beginning of the program, $\textrm{X} = x_I$, at
the end, $\textrm{X} = x_I + 2$, and along the way, $\textrm{X} = x_I+1$.

In this simple case, we have only three program states to consider, with no
real control flow. Suppose our program is instead:
\begin{algorithm}
  input:   An Integer $x_I$, assigned to X.
  output:  None
  begin
    if X > 4:
      X $\leftarrow$ X+1
    else:
      if X > 2:
        X $\leftarrow$ X+2
      else:
        X $\leftarrow$ X+3
    return
  end
\end{algorithm}
In this case, we have four states, and rather than occurring sequentially, they
branch. The branching, however, gives us some extra information. In addition to
knowing what symbolic values X assumes throughout the program, we know that, if
we find ourselves on the path that leads through line 5, then $x_I$ is greater
than four. If we find ourselves on the other path, $x_I$ is less than or equal
to four. 

So, the space of possible program states, their transitions, and our knowledge
on the constraints at each point looks like this:
\begin{center}
\begin{tikzpicture}[every node/.style={align=left, draw=black, outer sep=2pt,
  rounded corners=0.1cm}]
  \node (A) at (0,2) {X = $x_I$};
  \node (B) at (2,0) {X = $x_I+1$,\\ $x_I > 4$};
  \node (C) at (-2,0) {X = $x_I$,\\ $x_I \leq 4$ };
  \node (D) at (-1,-2) {X = $x_I+2$,\\ $x_I \leq 4$,\\ $x_I > 2$ };
  \node (E) at (-3,-2) {X = $x_I+3$,\\ $x_I \leq 4$,\\ $x_I \leq 2$ };

  \path [->] (A) edge (B);
  \path [->] (A) edge (C);
  \path [->] (C) edge (D);
  \path [->] (C) edge (E);
\end{tikzpicture}
\end{center}
In general, control flow that depends on the state of the program will introduce
similar branching. Because our knowledge increases as the symbolic execution
proceeds, it makes sense to visualize this process as the development of a tree,
rather than as a more general graph. Although we might return to the same
``program state'' in some sense, we generally will not return to the same state
with the same knowledge. 
% Can this be made more precise? Seems like this kind of return shouldn't be
% possible if the program is deterministic and terminates.

\toolname{} builds on the \angrname{} \cite{ANGR} binary analysis framework to explore ``all
possible paths'' through a program. In a nutshell, \toolname{} symbolically executes
two binaries, generating a complete tree of each binary's possible program
states and the transitions between them. It then uses the constraints that have
been discovered for each terminal symbolic state to determine, for each branch
$s$ from the symbolic execution tree of the pre-patch binary, which branches
$s'$ from the symbolic execution tree of the post-patch binary could occur under
conditions that would produce $s$. Section \ref{sec:comparative_analysis} will
explain this idea in more detail.

As a preview of what's to come, Figure \ref{fig:simple_symbolic_execution} displays how
\toolname{} visualizes the symbolic execution of a binary resulting from the
compilation of the facing c code.

\begin{figure}[h]\label{fig:simple_symbolic_execution}
  \begin{minipage}{0.2\textwidth}
  \includegraphics[width=0.9\textwidth]{cozy-2.png}
  \end{minipage}
  \begin{minipage}{0.2\textwidth}
  \begin{minted}{C}
  int main (int x) {
      if (x > 4) {
        x = x + 1
      } else if (x > 2) {
        x = x + 2
      } else {
        x = x + 3
      }
      return x;
  }
  \end{minted}
  \end{minipage}
  \caption{Symbolic execution of a simple binary}
\end{figure}


==> sections/extra.tex <==
Intro
=====
Patching legacy (deployed) software generally modifies only a small
portion of an overall software stack. Furthermore, it is often
difficult to recreate the original binary from sources, due to
toolchain ``bit rot'', and so updates to legacy software sometimes
must be implemented as binary-level patches. One can gain confidence
that a patch has made only the desired changes, and has not modified
previously correct behavior, by employing \emph{comparative binary
  analyses}: automated techniques for comparing the semantics of two
binary programs.

One such analysis is \emph{differential symbolic execution}, a technique that finds...
define differential symbolic execution
Execute programs on symbolic inputs, identify pairs of paths that are triggered by the same input, and then compare final states at the ends of those paths.

Differences in program behavior can be characterized in terms of differences between program states that are reachable by the same input.

One challenge of differential symbolic execution is interpreting the results.

The combination of large programs and path explosion, a well-known weakness of symbolic execution, can produce a large number of final states, and by extension, a large number of pairs of corresponding states. Knowing which pairs to filter out and which ones are patch-related is difficult.

Our tool, cozy\footnote{cozy on github:
\url{https://github.com/draperlaboratory/cozy}}, is a combination of
a symbolic evaluation and visualization interface that supports
analysis and exploration of micropatch modifications.

Since we are targeting a scenario where no source code is available,
we require an analysis framework capable of symbolically evaluating
binary programs. To achieve this, we have built our library on top
of the angr \cite{angr_paper} binary analysis platform.

\subsection{Aside: Benefits of Web Technologies}

\sml{This subsection can be deleted if we're over the page limit.}

As mentioned above, the \toolname{} GUI is implemented as a web application. The use of web technologies
in the \toolname{} development has several advantages:
%
\begin{itemize}
  \item The web ecosystem of libraries for data visualization and other
    UI niceties is immense. In particular, \toolname{} benefits from the
    use of cytoscapejs \cite{cytoscapejs} for graph visualization.
  \item The \toolname{} GUI is easily embeddable into any application that supports
    webviews. It is fairly straightforward to create simple plugins for, e.g.,
    VSCode or Ghidra that embed the GUI.
  \item Installation of the GUI is frictionless. It can be shipped as part of
    the \toolname{} Python package on PyPI, or bundled into a single HTML file.
    The GUI can also be used without any installation if
    accessed as part of a web page.
\end{itemize}


==> sections/supplemental_materials.tex <==
The \toolname{} framework is available as a Python package from PyPI via the \href{https://pypi.org/project/cozy-re/}{cozy-re} package. The source code is released under the MIT License and can be found at \url{https://github.com/draperlaboratory/cozy}. Documentation and tutorials can be found on our GitHub pages site at \url{https://draperlaboratory.github.io/cozy/}.

